Oracle-Supported Dynamic Exploit Generation for Smart Contracts

Despite the high stakes involved in smart contracts, they are often developed in an undisciplined manner, leaving the security and reliability of blockchain transactions at risk. In this paper, we introduce ContraMaster: an oracle-supported dynamic exploit generation framework for smart contracts. Existing approaches mutate only single transactions; ContraMaster exceeds these by mutating the transaction sequences. ContraMaster uses data-flow, control-flow, and the dynamic contract state to guide its mutations. It then monitors the executions of target contract programs, and validates the results against a general-purpose semantic test oracle to discover vulnerabilities. Being a dynamic technique, it guarantees that each discovered vulnerability is a violation of the test oracle and is able to generate the attack script to exploit this vulnerability. In contrast to rule-based approaches, ContraMaster has not shown any false positives, and it easily generalizes to unknown types of vulnerabilities (e.g., logic errors). We evaluate ContraMaster on 218 vulnerable smart contracts. The experimental results confirm its practical applicability and advantages over the state-of-the-art techniques, and also reveal three new types of attacks.

==> impl.tex <==
\section{Implementation and Optimizations}
\label{sec:impl}
%\lei{Add a summary Table on the problems, and issues that we could resolve}

==> overview.tex <==
\section{\tool Overview}
\label{sec:overview}

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.9\columnwidth]{figures/SimpleFlow.pdf}
% 	\caption{Overview of the \tool workflow.}\label{fig:SimpleFlow}
% \end{figure}

%\ca{The concrete example is too early/specific here (commented out). First, enough background 
%needs to be given.}

\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{figures/workflow/workflow.pdf}
  \caption{Overview of the \tool workflow.}\label{fig:workflow}
\end{figure}

Fig.~\ref{fig:workflow} shows the overview of \tool, which is driven by a grey-box fuzzing 
loop~\cite{listeelix,zalewski2016american}.
Given a set of initial seeds, \tool randomly synthesizes a set of call sequences and picks one from 
the pool in each iteration of the fuzzing loop.
\tool runs each transaction in sequence on an instrumented EVM.
When the transaction is finished, \tool verifies the contract state against our \emph{semantic test 
oracle} (details in Sect.~\ref{subsec:Oracle}).
If a violation is detected, \tool reports a vulnerability and presents the generated attack 
contract and transaction sequence which can be used to reproduce the exploit.
Otherwise, \tool collects runtime execution information to guide the test sequence generation for 
the next iteration.
The information collected mainly includes the control flow graph (CFG) edge coverage and the 
commonly seen dictionary values.

%In the execution information of each call, \tool performs control-flow analysis towards CFG edge 
%coverage, and contract state analysis to extract the dynamic dictionary information.
%In the total execution information of call sequence, \tool conducts data-flow analysis to guide 
%call sequence mutation (c.\,f.~Sect.~\ref{subsec:feedback}).

Furthermore, \tool is equipped with a number of new mutation operators customized for smart 
contracts (c.\,f.~Sect.~\ref{subsec:Mutation}).
In addition to \emph{function inputs} used in fuzzing of traditional computer programs, we also use 
\emph{gas limits}, \emph{fallback functions}, \emph{transaction sequences} and \emph{contract 
states} as the mutation targets.
Many vulnerabilities in smart contracts require the interplay of several contracts and can only be 
exploited by a particular transaction sequence with the correct gas limit~\cite{Kolluri2018Law}.
Therefore, the customized mutation operators are important for generating effective test inputs.
The newly generated inputs are added to the pool and the fuzzing process continues until it exceeds 
the allocated resource limits.

%\subsection{Attack Scenarios}
%Unlike in general computer programs, some vulnerabilities in smart contracts (e.g., reentrancy and 
%exception disorder) happen between several contracts.
%To this end, \tool needs to automatically synthesize the attack contracts to start the fuzzing 
%process, an example is shown in Fig.~\ref{fig:reentrancy}.
%In the fuzzing process, we use attack contracts to start a transaction and interact with target 
%contracts.

\paragraph{\tool by Example}
Take the DAO contract in Fig.~\ref{fig:dao} as an example.
Based on the initial seeds \{\textit{withdraw(10)}, \textit{deposit.value(5)(*)}\}, \tool randomly 
synthesizes a transaction sequence, ``$\mathit{ts}_1$ = \textit{withdraw(10)} $\rightarrow$ 
\textit{deposit.value(5)(*)}''.
After $\mathit{ts}_1$ is executed, we identify a data dependency between \textit{withdraw} and 
\textit{deposit} over the state variable \textit{balances} by analyzing the data flow of the 
execution trace.
Using this as feedback, we mutate $\mathit{ts}_1$ and generate ``$\mathit{ts}_2$ =  
\textit{deposit.value(5)(*)} $\rightarrow$ \textit{withdraw(10)}''. 
In $\mathit{ts}_2$'s execution, we assume it does not produce the reentrancy, because the value 
withdrawn is greater than that deposited.
In addition, \tool extracts the contract states as the dynamic dictionary, e.g., the amount 
deposited into \textit{balances} is 5.
Next, \tool randomly generates three group of inputs (less than 5, 5, great than 5) as the 
parameter of \textit{withdraw}, e.g., we get ``$\mathit{ts}_3$ =  \textit{deposit.value(5)(*)} 
$\rightarrow$ \textit{withdraw(3)}''.
At present, we still assume the reentrancy does not happen, because the attack contract may not 
contain the right fallback function, e.g., \textit{another\_attackDAO} in Fig.~\ref{fig:exception}.
Since \tool also performs the mutation on fallback function, and thus may generate new fallback 
function, as \textit{attackDAO} in Fig.~\ref{fig:reentrancy}.
Finally, we have \textit{attackDAO} in Fig.~\ref{fig:reentrancy} as attack contract, and execute 
``\textit{deposit.value(5)(*)} $\rightarrow$ \textit{withdraw(3)}'', it would trigger the 
reentrancy.

%In a normal transaction, the amount deducted from the externally visible balance (i.e., 
%\textit{this.balance}) should be reflected as the same amount deducted from the internal 
%bookkeeping (i.e., \textit{balances} at Line 2 in Fig.~\ref{fig:dao}).
When the reentrancy takes place, \ether would be transferred to the attacker's account via the 
\textit{withdraw} function, but without updating \textit{balances} at Line 9 due to gas limit.
Since the value of bookkeeping variable \textit{balances} is wrong, and thus our balance invariant 
is violated.

